Optimal Data Acquisition with Privacy-Aware Agents

We study the problem faced by a data analyst or platform that wishes to collect private data from privacy-aware agents. To incentivize participation, in exchange for this data, the platform provides a service to the agents in the form of a statistic computed using all agents' submitted data. The agents decide whether to join the platform (and truthfully reveal their data) or not participate by considering both the privacy costs of joining and the benefit they get from obtaining the statistic. The platform must ensure the statistic is computed differentially privately and chooses a central level of noise to add to the computation, but can also induce personalized privacy levels (or costs) by giving different weights to different agents in the computation as a function of their heterogeneous privacy preferences (which are known to the platform). We assume the platform aims to optimize the accuracy of the statistic, and must pick the privacy level of each agent to trade-off between i) incentivizing more participation and ii) adding less noise to the estimate. We provide a semi-closed form characterization of the optimal choice of agent weights for the platform in two variants of our model. In both of these models, we identify a common nontrivial structure in the platform's optimal solution: an instance-specific number of agents with the least stringent privacy requirements are pooled together and given the same weight, while the weights of the remaining agents decrease as a function of the strength of their privacy requirement. We also provide algorithmic results on how to find the optimal value of the noise parameter used by the platform and of the weights given to the agents.

==> incentives.tex <==
\section{On Strategic Agents and Misreporting Costs}
Up until now, we have considered a setting in which the privacy costs of the agents are known to the platform. However, in practice, the platform may have to elicit said privacy costs from the agents. In such situations, agents may lie about their costs to get better outcomes, and we need to make sure that our approach incentivizes truthful reporting. We note that the follow-up work of \cite{ec2022} shows how to design truthful mechanisms under our ``quasi-linear'' agent model, hence we focus on the ``privacy-constrained'' model in this section. 

% The analyst's direct revelation mechanism we consider is then the following:
% \begin{enumerate}
% \item The analyst asks each agent $i$ to report $\tau_i$. Agent $i$ reports $\hat{\tau}_i$ that may differ from $\tau_i$ if it is in his best interest to misreport.
% \item The analyst collects the agents' reports $\hat{\tau}_1, \ldots, \hat{\tau}_n$, and announces the solution $(\w,\eta)$ to Program~\eqref{eq:optim_threshold}. 
% \item Each agent $i$ decides whether he wants to participate given $w_i, \eta$.
% \item Finally, the analyst runs estimator $\hat{\theta} = \sum_{i \in S} w_i x_i + L(\eta)$ on the participating agents.
% \end{enumerate}


% \begin{clm}
% For every agent $i$, reporting $\hat{\tau}_i < \tau_i$ is a (weakly) dominated strategy.
% \end{clm}
% I.e., agents do not report privacy preferences that are \emph{more} stringent than their true privacy preferences. The idea is that doing so makes the analyst's problem harder, which leads to higher variance and in turn a worse utility for each agent. 

% \begin{proof}
% Fix the report $\hat{\tau}_{-i}$ of the remaining agents. Suppose agent $i$ reports $\hat{\tau_i} < \tau_i$. We have two cases:
% \begin{enumerate}
% \item Program \eqref{eq:optim_simpler_model} is infeasible, or the solution of Program \eqref{eq:optim_simpler_model} is such that $c_i w_i \eta > B_i$. Then $i$ decides not to participate and gets utility $0$, while reporting the truth would have led to non-negative utility for agent $i$.
% \item Otherwise, note that since for agent $i$, $c_i w_i \eta < \hat{c}_i w_i \eta \leq B_i$, it immediately follows that 
% \[
% Var^*(c_i,\hat{\cost}_{-i}) \leq Var^*(\hat{c}_i,\hat{\cost}_{-i}),
% \]
% noting that the right-hand-side optimization program has a strictly smaller feasible set. In turn, reporting $\hat{c}_i > c_i$ cannot decrease the variance of the analyst's estimate hence increase agent $i$'s utility.
% \end{enumerate}
% This concludes the proof.
% \end{proof}



\paragraph{A note on agent incentives} Now, let us suppose that each agent $i$, on top of deciding whether to participate, can also strategically misreport their threshold $\tau_i$ in order to increase his utility. We now consider the following interactions between the platform and the agents:
\begin{enumerate}
    \item Each agent $i$ decides whether to join the platform, and what privacy threshold $\htau_i$ to report. Note that $\htau_i$ may be different from $\tau_i$ if it is in the agent's best interest to do so. 
    \item The platform solves 
    \begin{align}
    \begin{split}\label{eq:optim_strategic}
    \min_{\w,\eta}~& \sum_{i =1}^n w_i^2 \sigma^2 + \frac{2}{\eta^2}
    \\\text{s.t.}~& w_i \eta \leq \htau_i~~\forall i \in [n]
    \\& \sum_{i = 1}^n w_i = 1
    \\&w_i \geq 0~\forall i.
    \end{split}
    \end{align}
    \item Let $(\w,\eta)$ be the solution to Program~\ref{eq:optim_strategic}. Each agent $i$ gets utility $\sum_i w_i^2 + \frac{2}{\eta}$ if $w_i \eta \leq \tau_i$, and $-\infty$ otherwise. Note that an agent can obtain $-\infty$ utility if they decide to participate but use a sub-optimal report $\htau_i$. 
\end{enumerate}

Here, we remark that our mechanism has nice incentive properties. First, we show that all agents join the platform.
\begin{itemize}
    \item 
\end{itemize}
